A Closed-Form Solution to Local Non-Rigid Structure-from-Motion

A recent trend in Non-Rigid Structure-from-Motion (NRSfM) is to express local, differential constraints between pairs of images, from which the surface normal at any point can be obtained by solving a system of polynomial equations. The systems of equations derived in previous work, however, are of high degree, having up to five real solutions, thus requiring a computationally expensive strategy to select a unique solution. Furthermore, they suffer from degeneracies that make the resulting estimates unreliable, without any mechanism to identify this situation. In this paper, we show that, under widely applicable assumptions, we can derive a new system of equation in terms of the surface normals whose two solutions can be obtained in closed-form and can easily be disambiguated locally. Our formalism further allows us to assess how reliable the estimated local normals are and, hence, to discard them if they are not. Our experiments show that our reconstructions, obtained from two or more views, are significantly more accurate than those of state-of-the-art methods, while also being faster.

==> tex/mbkg.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\subsection{NRSfM Formalism}

Recall from Section~\ref{sec:outline} and Fig.~\ref{fig:model} that we are given an image registration function $\eta$ that associates points in the first image $\mathcal{I}$ to points in the second $\overline{\mathcal{I}}$ and we want to infer from it the functions $\phi , \overline{\phi}: \mathbb{R}^2 \to \mathbb{R}^3$ that associate a surface point to an image point. 

Given a point $\mathbf{x} = (u,v)$ on $ \mathcal{I}$ and its corresponding 3D point $\mathbf{X} = \phi(\mathbf{x})$  on $ \mathcal{S}$, we write $\phi(\mathbf{x})=\frac{1}{\beta(u,v)}\begin{pmatrix}
u & v & 1 \end{pmatrix}^\top$, where $\beta$ is a linear function that represents the inverse of depth. \PF{Why is $\beta$ linear?} The Jacobian of $\phi$ is given by
%
\begin{equation}
\label{eq:j_phi}
  \mathbf{J}_\phi = \frac{1}{\beta(u,v)}\begin{pmatrix}
1- uk_1 & -uk_2 \\ -vk_1 & 1-vk_2 \\ -k_1 & -k_2
\end{pmatrix},
\end{equation}
%
where  $k_1=\frac{\partial_u \beta}{\beta}$ and $k_2=\frac{\partial_v \beta}{\beta}\right)$.  $\overline{u}$, $\overline{v}$, $\overline{\phi}$,  $\overline{k_1}$, and   $\overline{k_2}$ are defined similarly in $\overline{\mathcal{I}}$.
 
 %= \frac{1}{\beta(u,v)}\hat{\mathbf{x}}
 
\parag{Metric Tensors.} 

The metric tensors $\mathbf{g}$ in $ \mathcal{I}$ and $\overline{\mathbf{g}}$ in $\overline{\mathcal{I}}$ are first-order differential quantity that capture local distances and angles. They can be written as
%
 \begin{equation}
\mathbf{g}=\mathbf{J}_\phi^\top\mathbf{J}_\phi \text{ and } \overline{\mathbf{g}}=\mathbf{J}_{\overline{\phi}}^\top \mathbf{J}_{\overline{\phi}} \; .
 \end{equation}
%
These tensors can be used to imposed to impose isometric, conformal, and equiareal constraints by forcing the scalars $k_1$ and $k_2$ of Eq.~\ref{eq:j_phi} to satisfy one of the three conditions below:
%
\begin{equation}
\label{eq:iso-nrsfm}
%\text{Find }(k_1,k_2)\text{ s.t. }\!
\begin{cases}
\overline{\mathbf{g}}\!=\!\mathbf{J}_\eta^\top \mathbf{g}\mathbf{J}_\eta,\!&\!\text{Isometry} 
\\
\overline{\mathbf{g}}\!=\!\lambda^2\mathbf{J}_\eta^\top \mathbf{g}\mathbf{J}_\eta, \! \lambda^2\!\in\!\mathbb{R}^{+}\! -\! {1},\!&\!\text{Conformality} 
\\
\det(\overline{\mathbf{g}})\!=\!\det(\mathbf{J}_\eta^\top \mathbf{g}\mathbf{J}_\eta),\!&\!\text{Equiareality} 
\end{cases}
\end{equation}
%



\parag{Connections.} 

Connections are second-order differential quantities that express the rate of change of the metric tensors. \pf{Under the assumption of local linearity, it can be shown~\cite{Parashar19a}} that
%
\begin{equation}
\label{eq:CS_rel}
\begin{pmatrix}
\overline{k}_1 \\ \overline{k}_2
\end{pmatrix} = \mathbf{J}_\eta^\top\begin{pmatrix}
k_1 \\ k_2
\end{pmatrix} -\begin{pmatrix}
0 & 1 \\ 1 & 0
\end{pmatrix}\mathbf{J}_\eta^{-1}\dfrac{\partial^2 \eta}{ \partial \overline{u}\overline{v}} .
\end{equation}
%
The solutions to isometric, conformal and equiareal NRSfM are obtained by solving the metric tensor preservation equations of Eq.~\eqref{eq:iso-nrsfm} under the constraint  of Eq.~\eqref{eq:CS_rel}.

%--------
% OLD
%--------



%~\cite{Parashar19a} finds a common solution to isometric and conformal NRSfM. It obtains  a pair of cubic equations in terms of $(k_1,k_2)$ and solve them by minimising the sum-of-squares of the equations obtained over multiple image-pairs. According to B\'ezout's theorem, there are 9 possible solutions to this system of equations.~\cite{Parashar20a} demonstrates that there are 9 possible structures of these equations and proves that there exists at least one real  solution to each of these structures. It is difficult to comment whether the equations represent a non-degenerate data or not. Therefore, it is impossible to argue that the equations are well-posed. \PF{Again do we need this paragraph here?}





==> tex/outline.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\section{Method Framework}
\label{sec:outline}

\input{fig/model}

Fig~\ref{fig:model} depicts our setup when using only two images $\mathcal{I}$ and $\overline{\mathcal{I}}$ acquired by a calibrated camera. In each one, we denote the deforming surface as $\mathcal{S}$  and $\overline{\mathcal{S}}$, respectively, and model it  in terms of functions $\phi , \overline{\phi}: \mathbb{R}^2 \to \mathbb{R}^3$ that associate a surface point to an image point. Let us assume that we are given an image registration function $\eta: \mathbb{R}^2 \to \mathbb{R}^2$ that associates points in the first image to points in the second. In practice, it can be computed using standard image matching techniques such as optical flow~\cite{Sundaram10,Sun18a} or SIFT~\cite{Lowe04}. These functions can be composed to create a mapping $\psi: \mathbb{R}^3 \to \mathbb{R}^3$ from 3D surface points seen in the two images. We use a parametric representation of $\eta$ and $\phi$ using thin-plate splines~\cite{Bookstein89}, which allows us to accurately obtain first-order derivatives of these functions. A finite-difference approach could also be used.

At the heart of our approach is the fact, which we will prove, that the normals at two corresponding points can be computed from $\eta$ and $\phi$ under the sole assumptions of local planarity and local linearity. \PF{Explain!}


%\ShP{We have two assumptions here: A) sufaces are locally planar and B) deformations are locally linear. Without local linearity of deformations, we cannot write connections the way we normally do. esxcept for isometry.} %\MS{What does this mean?} \shp{Therefore, if we take $\mathcal{I}$ to be the reference image  in which we wish to recover the shape, we can write the constraints with as many images $\overline{\mathcal{I}}$ to increase the number of points of  $\mathcal{S}$ for which we have normals and recover the shape of $\mathcal{S}$ by integration, with the cost only growing linearly with the number of images being used.}
%\ShP{This sentence is indeeed confusing. All we want to say is that in order to construct normals, we consider each point correspondence independently. After we have obtained normals for each surface, we obtain depth by integrating the normals of each surface.} \MS{This paragraph is strange. Do you use different $\overline{\mathcal{S}}$ or different points from $\overline{\mathcal{S}}$?} The shape of all $\overline{\mathcal{S}}$ can then be expressed in terms of the recovered shape at $\mathcal{S}$. \MS{And why is this important?} \ShP{So that we sont have to redo the experiment for each shape seperately. We take one as reference, reconstruct it, and thanks to the  connections we reconstruct the normals on other surfaces using the normals at reference surface. ~\cite{Chhatkuli14} and~\cite{Varol09} reconstrct only the reference image. So, in order to reconstruct N surfaces, they have to run their method N times.  }

The earlier methods~\cite{Parashar19a,Parashar20a} rely on a similar formalism, but our approach has two key advantages: 
%
\begin{enumerate}

\item The system of equations we solve to compute the normals only has at most two solutions, instead of five when the system is expressed in terms of depth derivatives as  in~\cite{Parashar19a,Parashar20a}. In practice, we pick the solution that minimizes the sum of squares of depth derivatives. In other words, we choose the normals that correspond to the smallest depth-change, thus promoting smoothness.

\item Given that not all motions are conducive to reliable normal estimates,  our formulation enables us to explicitly quantify which normals can be trusted because the system of equations used to derive them was well-conditioned and which cannot. Hence, when integrating the normals to recover the 3D surfaces, we can discard the untrustworthy ones, which as we will see in the result section gives us a significant performance boost. 

\end{enumerate}
%
\comment{
As in~\cite{Parashar20a}, we assume the deformations to be diffeomorphic but with two main differences:
\begin{enumerate}

 \item  We assume the surfaces to be infinitesimally planar instead of infinitesimally linear. This means that the second second-order derivatives can be expressed in terms of the first-order ones but are non-zero. \PF{Correct?}. \ShP{Yes}
 

 \item  In~\cite{Parashar20a} the diffeomorphic constraints are expressed solely in terms of connections \MS{We have not mentioned anything about connections so far. This will not be clear to the reader.} and the metric tensor is only used to enforce additional constraints, such as isometry, conformality or equiareality. By contrast, we use both the metric tensor and the connections and show that all possible deformation types are represented by only one constraint. \MS{This discussion is quite obscure to me. Is it really the right place to have this entire paragraph?} \PF{I find Mathieu's comment reassuring. I have absolutely no idea what this paragraph means ;-)} \ShP{I will take this paragraph as a discussion in the end of the paper}
 \end{enumerate}
 }
%One drawback, however, is that we have to assume a local isometry unlike the method of~\cite{Parashar20a}, which only requires the local deformations to be diffeomorphic. We will demonstrate, that in practice, our method tolerates local extensions, which makes it applicable to a wide range of objects.

%At the heart of our approach is the fact that, under the assumption that the two surfaces are locally diffeomorphic, some differential properties of corresponding 3D points should match. These properties can be expressed in terms of {\it connections}. They are generic properties of a differentiable surface that express intrinsic relationship between a point on the surface and its local neighborhood~\cite{Cartan23,Ivey16}. In particular, the well known first and second fundamental forms on surfaces can be derived from them. Crucially, they are preserved under diffeomorphism~\cite{Parashar19a}, which we prove formally. Furthermore, assuming the surfaces to be locally planar, we show that we can use connections computed using {\it only} first derivatives. Thus, we can express depth and its derivatives at $\overline{\mathcal{S}}$ in terms of the same quantities at $\mathcal{S}$. As a consequence, the 3D coordinates of corresponding points on the surface are strongly constrained, thanks to multi-view constraints and the 3D reconstruction problem becomes sufficiently constrained. This approach has several strengths: 
%
%\begin{itemize}
% \item Because all the constraints can be expressed in terms of first derivatives of $\phi$, $\overline{\phi}$ and $\eta$, which, unlike the second derivatives that are required by the formulation of~\cite{Parashar19a}, can be estimated even if the points for which we have correspondences are relatively sparse.  
% \item If we happen to know that the deformation is isometric, conformal, or equiareal, we can easily incorporate these additional constraints into our framework.
% \item If we take $\mathcal{S}$ to be the reference image in which we wish to recover the shape, we can write the constraints for as many surfaces $\overline{\mathcal{S}}$ as we want to increase robustness and the cost only grows linearly with the number of such images. The shape at $\overline{\mathcal{S}}$ can then be expressed in terms of the recovered shape at $\mathcal{S}$.
%\end{itemize}
%%
%We now define connections  and then show their usage. 




==> tex/reform.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\section{Computing Normals from Two Images}

In earlier approaches the  NRSfM problem was addressed by solving the system of equations of~\ref{eq:nrsfm} under the isometric, conformal, and equiareal constraints of Eq.~\ref{eq:iso-nrsfm} with respect the variables $k_1$ and $k_2$ of Eq.~\ref{eq:j_phi}. In our approach, we solve the system of equations directly in terms of the surface normals. We do this in  closed form while simultaneously identifying degenerate conditions that result in unreliable estimates. 


\parag{Differentiating the Warp.}

Let us consider a point $\overline{\mathbf{x}} = (\overline{u},\overline{v})^T$ in $\overline{\mathcal{I}}$ and its corresponding point $(u,v)^T=\eta(\overline{u},\overline{v})$  in  $\mathcal{I}$. Assuming the surfaces to be infinitesimally planar means that there is a $3 \times 3$ homography matrix $\mathbf{H} = [h_{ij}]_{1 \leq i,j \leq 3}$ relating $\overline{\mathbf{x}}$ and $\mathbf{x}$. Assuming the homography to be normalized, that is, its second singular value to be 1, we write
\begin{equation}
\label{eq:homography}
\!\begin{pmatrix}
u \\ v \\ 1
\end{pmatrix}\!=\!\frac{1}{\overline{s}}\!\begin{pmatrix}
h_{11} \!& \!h_{12} \!&\! h_{13} \\
h_{21} \!&\! h_{22} \!&\! h_{23} \\
h_{31} \!&\! h_{32} \!&\! h_{33} 
\end{pmatrix}\!\begin{pmatrix}
\overline{u} \\ \overline{v} \\ 1
\end{pmatrix}, \; 
\end{equation} 
where $\overline{s}=h_{31}\overline{u}\!+\!h_{32}\overline{v}\!+\!h_{33}$.  Thus the first and second-order derivatives of $\eta$ can be computed as 
\begin{align}
\label{eq:eta_der}
\begin{pmatrix}
\dfrac{\partial \eta}{\partial \overline{u}} & \dfrac{\partial \eta}{\partial \overline{v}}
\end{pmatrix}&=\frac{1}{\overline{s}}
\begin{pmatrix}
h_{11}\!-\!h_{31}u \!&\! h_{12}\!-\!h_{32}u \\
h_{21}\!-\!h_{31}v \!&\! h_{22}\!-\!h_{32}v
\end{pmatrix} = \mathbf{J}_\eta \; , \nonumber \\[1mm]
\begin{pmatrix}
\dfrac{\partial^2 \eta}{ \partial \overline{u}^2} & \dfrac{\partial^2 \eta}{ \partial \overline{u}\overline{v}} & \dfrac{\partial^2 \eta}{ \partial \overline{v}^2}
 \end{pmatrix} 
&= -\frac{1}{\overline{s}} \mathbf{J}_\eta\begin{pmatrix}
2h_{31} & h_{32} & 0 \\ 0 & h_{31} &2h_{32}
\end{pmatrix}.
\end{align}

\parag{Image Embedding and Local Normal.}

The unit normal $\mathbf{n}$ at $\mathbf{x}$ is the cross product of the columns of  the matrix $\mathbf{J}_\phi$ from~Eq.~\ref{eq:j_phi}. We write
%
\begin{align}
\label{eq:normal}
\mathbf{n} & =\! \frac{1}{\beta^2\sqrt{\det \mathbf{g}}}\!\begin{pmatrix}
k_1 \\k_2 \\ 1\!-\!uk_1\!-\!vk_2
\end{pmatrix} \\
%
&=\!\frac{1}{\beta^2\sqrt{\det \mathbf{g}}}\!\begin{pmatrix}
\mathbf{I}_{2\times 2} & 0 \\ -\mathbf{x}^\top &1
\end{pmatrix}\!\begin{pmatrix}
k_1 \\ k_2 \\ 1
\end{pmatrix}\!. \nonumber \\
%
\Rightarrow 
\begin{pmatrix}
k_1 \\ k_2 \\ 1
\end{pmatrix} & =\!\beta^2\sqrt{\det \mathbf{g}}\begin{pmatrix}
\mathbf{I}_{2\times 2} & 0 \\ \mathbf{x}^\top &1
\end{pmatrix}\mathbf{n}. \label{eq:k1k2}
\end{align}
%
Given the normal $\mathbf{n}$ as written in Eq.~\ref{eq:normal}, we re-write the matrix $\mathbf{J}_\phi$ of Eq.~\ref{eq:j_phi} as
%
\begin{align}
\label{eq:j_phi_in_n}
\nonumber
\mathbf{J}_\phi \!&\!=\! \beta\sqrt{\det \mathbf{g}}\!\begin{pmatrix}
0 &  uk_1\!+\!vk_2\!-\!1 & k_2 \\
1\!-\!uk_1\!-\!vk_2 & 0 & \!-\!k_1 \\
\!-\!k_2 & k_1 & 0
\end{pmatrix}\!
\begin{pmatrix}
0 & 1 \\ \!-\!1 & 0 \\ v & \!-\!u
\end{pmatrix} \\
\!&\!=\! \beta\sqrt{\det \mathbf{g}}[\mathbf{n}]_{\times}\mathbf{E}.
\end{align}
%
We can now rewrite the differential constraints across images introduced in Section~\ref{sec:diffConstraints}  in terms of the normals.

\parag{Connections.} 

Given the $\eta$ derivatives~Eq.\ref{eq:eta_der}, the connections transfer relation of Eq.~\ref{eq:CS_rel} becomes
%
\begin{align}
\label{eq:CS_law}
\begin{pmatrix}
\overline{k}_1 \\ \overline{k}_2
\end{pmatrix}&=\!\mathbf{J}_\eta^\top\!\begin{pmatrix}
k_1 \\ k_2
\end{pmatrix}\!+\!\dfrac{1}{\overline{s}}\!\begin{pmatrix}
h_{31} \\h_{32}
\end{pmatrix} \; , \nonumber \\
\Rightarrow
\begin{pmatrix}
\overline{k}_1 \\ \overline{k}_2 \\ 1
\end{pmatrix}&=\!\begin{pmatrix} 
\mathbf{J}_\eta^\top & \mathbf{m} \\ 0 & 1 \end{pmatrix}\!\begin{pmatrix}
k_1 \\k_2 \\1
\end{pmatrix}\!. 
\end{align}
Using Eq.~\ref{eq:k1k2}, we re-write the above expression  as
%
\begin{align}
\label{eq:CS_norm}
\nonumber
\overline{\mathbf{n}}\!&\!=\!\frac{\beta^2}{\overline{\beta}^2}\!\sqrt{\frac{\det \mathbf{g}}{\det \overline{\mathbf{g}}}}\mathbf{T}\mathbf{n}\\
\nonumber  \!&\!=\!\frac{\beta^2}{\overline{\beta}^2}\!\sqrt{\frac{\det \mathbf{g}}{\det \overline{\mathbf{g}}}}\!\begin{pmatrix}
\mathbf{I}_{2\times 2} & 0 \\ -\overline{\mathbf{x}}^\top &1
\end{pmatrix}\!\begin{pmatrix} 
\!\mathbf{J}_\eta^\top\!&\!\mathbf{m}\!\\ 0 & 1 \end{pmatrix}\!\begin{pmatrix}
\!\mathbf{I}_{2\times 2}\!&\!0\!\\ \mathbf{x}^\top &1
\end{pmatrix}\!\mathbf{n}
\\ \nonumber
\!&\!=\!\dfrac{ \beta^2}{\overline{s}\overline{\beta}^2}\!\sqrt{\frac{\det\!\mathbf{g}}{\det\!\overline{\mathbf{g}}}}\!\begin{pmatrix}
\!\mathbf{I}_{2\times 2}\!&\!0\!\\\!-\!\overline{\mathbf{x}}^\top\!&\!1\!
\end{pmatrix}\!\begin{pmatrix}
\!h_{11}\!&\!h_{21}\!&\!h_{31}\!\\
\!h_{12}\!&\!h_{22}\!&\!h_{32}\!\\
\!\overline{s}u\!&\!\overline{s}v\!&\!\overline{s}\!
\end{pmatrix}\!\mathbf{n}\! \\ &\!=\!\dfrac{ \beta^2}{\overline{s}\overline{\beta}^2}\sqrt{\frac{\det\!\mathbf{g}}{\det\!\overline{\mathbf{g}}}}\!\mathbf{H}^\top\!\mathbf{n} \; ,
\end{align}
which directly relates the two normals.

\parag{Metric Tensor.}

As can be seen in Fig.~\ref{fig:model}, we can write $\overline{\phi} = \psi \circ \phi \circ \eta$. Differentiating this expression and multiplying it by its transpose yields
%
\begin{equation}
\label{eq:mt_gen}
\overline{\mathbf{g}}=\mathbf{J}_{\overline{\phi}}^\top\mathbf{J}_{\overline{\phi}} = \mathbf{J}_\eta^\top\mathbf{J}_\phi^\top\mathbf{J}_\psi^\top\mathbf{J}_{\psi}\mathbf{J}_\phi\mathbf{J}_\eta.
\end{equation}
%
For isometric, conformal and equiareal deformations, the matrix $\mathbf{J}_\psi^\top\mathbf{J}_\psi$ is given by $\mathbf{I}_{3\times3}$, $\lambda^2\mathbf{I}_{3\times3}$ and $diag(\lambda^2_1, \lambda^2_2,(\lambda_1\lambda_2)^{-2})$, where $\lambda_1^2,\lambda_2^2 \in \mathbb{R}^{+}$, respectively which leads to the  metric preservation relations of Eq.~\ref{eq:iso-nrsfm}.

When the deformation is diffeomorphic, $\mathbf{J}_\psi$ has 9 degrees of freedom. Using SVD, we write $\mathbf{J}_\psi = \mathbf{U} \Sigma \mathbf{V}^\top$, where $\mathbf{U}, \mathbf{V}$ are two orthogonal matrices and $\Sigma$ is a diagonal matrix. Therefore, $\mathbf{J}_\psi^\top\mathbf{J}_\psi = \mathbf{V}\Sigma^\top\Sigma\mathbf{V}^\top$. Since $\mathbf{V}$ is orthogonal, we can simplify Eq.~\eqref{eq:mt_gen}  as
%
\begin{equation}
\label{eq:mt_gen_simp}
\overline{\mathbf{g}} = trace(\Sigma^\top\Sigma)\mathbf{J}_\eta^\top \mathbf{g} \mathbf{J}_\eta = \sigma^2\mathbf{J}_\eta^\top \mathbf{g} \mathbf{J}_\eta.
\end{equation}
%
Thus, the different conditions of Eq.~\ref{eq:iso-nrsfm} combined into one single diffeomorphic constraint.

We now use Eq~\eqref{eq:j_phi_in_n} to rewrite the metric  preservation relation of Eq.~\eqref{eq:mt_gen_simp} as
%
\begin{small}
\begin{align}
\label{eq:mt_norm}
\!\overline{\beta}^2\!\det\!(\overline{\mathbf{g}})\overline{\mathbf{E}}^\top\![\overline{\mathbf{n}}]_\times^\top\![\overline{\mathbf{n}}]_\times\!\overline{\mathbf{E}}\!=\!\sigma^2\!\beta^2\!\det\!(\mathbf{g})\!\mathbf{J}_\eta^\top\!\mathbf{E}^\top\![\mathbf{n}]_\times^\top\![\mathbf{n}]_\times\!\mathbf{E}\!\mathbf{J}_\eta.
\end{align}
\end{small}
%
Given the $\eta$ derivatives of Eq-\eqref{eq:eta_der}, we simplify $\mathbf{E}\mathbf{J}_\eta$ to $\frac{1}{\overline{s}}\begin{pmatrix}
\mathbf{h}_1 \times \hat{\mathbf{x}} & \mathbf{h}_2 \times \hat{\mathbf{x}}
\end{pmatrix}$ where $\mathbf{h}_1, \mathbf{h}_2$ are the two columns of $\mathbf{H}$~\eqref{eq:homography}. By writing $\mathbf{z}_1 = \mathbf{n} \times (\mathbf{h}_1 \times \hat{\mathbf{x}})$ and $\mathbf{z}_2 = \mathbf{n} \times (\mathbf{h}_2 \times \hat{\mathbf{x}})$, Eq.~\eqref{eq:mt_norm} reduces to
%
\begin{small}
\begin{equation}
\label{eq:mt_norm_simp}
\overline{\beta}^2\det (\overline{\mathbf{g}})\overline{\mathbf{E}}^\top[\overline{\mathbf{n}}]_\times^\top[\overline{\mathbf{n}}]_\times\overline{\mathbf{E}} \! = \! \frac{\sigma^2\beta^2\det (\mathbf{g})}{\overline{s}^2}\begin{pmatrix}
\mathbf{z}_1^\top \mathbf{z}_1 \!\! & \!\! \mathbf{z}_1^\top \mathbf{z}_2 \\ \mathbf{z}_1^\top \mathbf{z}_2 \!\! &\!\! \mathbf{z}_2^\top \mathbf{z}_2 
\end{pmatrix} \! .
\end{equation}
\end{small}
%

\parag{Diffeomorphic NRSfM.} 

\pf{ So far, we have expressed the metric preservation conditions in terms of the normals of the two surfaces under consideration. The only unknown left in the system is therefore, $\mathbf{n}$. Hence, we now derive a closed-form solution} to diffeomorphic NRSfM by solving these equations in a closed-form. }

%Next we use Eq.~\ref{eq:CS_norm} to simplify the above expression by expressing $\overline{\mathbf{n}}$ in terms of $\mathbf{n}$.

Given the multiplication property of the cross product, the constraints on the normals of Eq.~\ref{eq:CS_norm} imply that  
%
\begin{equation}
[\overline{\mathbf{n}}]_\times=\dfrac{\gamma \beta^2}{\overline{s}\overline{\beta}^2}\sqrt{\frac{\det\mathbf{g}}{\det\overline{\mathbf{g}}}}\det (\mathbf{H}^\top) \mathbf{H}^{-1}[\mathbf{n}]_\times \mathbf{H}^{-\top} \; ,
\end{equation}
%
which lets us rewrite as the matrix $\mathbf{J}_{\overline{\phi}}$ of Eq.~\eqref{eq:j_phi_in_n} as
%
\begin{align}
\label{eq:jphi_n_overline}
\nonumber
\mathbf{J}_{\overline{\phi}}&\!=\!\frac{ \beta^2}{\overline{\beta}}\sqrt{\det \mathbf{g}} \mathbf{H}^{-1}\![\mathbf{n}]_\times\!\left(\!\frac{\det \mathbf{H}^\top}{\overline{s}}\!\mathbf{H}^{-\top}\overline{\mathbf{E}}\!\right)
\\
&\!=\!\frac{\ \beta^2\!\sqrt{\det \mathbf{g}}}{\overline{\beta}}\!\mathbf{H}^{\!-1}\![\mathbf{n}]_\times\!\begin{pmatrix}
\!\mathbf{h}_1\!\times\!\hat{\mathbf{x}}\!&\!\mathbf{h}_2\!\times\!\hat{\mathbf{x}}\!\end{pmatrix} \\ \nonumber
&\!=\!\frac{ \beta^2\!\sqrt{\det \mathbf{g}}}{\overline{\beta}}\!\mathbf{H}^{\!-1}\!\begin{pmatrix}
\!\mathbf{z}_1\!&\!\mathbf{z}_2\!
\end{pmatrix}\!.
\end{align}
%
Injecting this expression into  the metric tensor preservation relation of Eq.~\ref{eq:mt_norm_simp} yields
%
\begin{small}
\begin{align}
\label{eq:recon_eqn}
\begin{pmatrix}
\mathbf{z}_1^\top\mathbf{H}^{\!-\top}\!\mathbf{H}^{\!-\!1} \mathbf{z}_1\!&\!\mathbf{z}_1^\top\mathbf{H}^{\!-\!\top}\!\mathbf{H}^{\!-\!1} \mathbf{z}_2\! \\ \mathbf{z}_1^\top\mathbf{H}^{\!-\!\top}\!\mathbf{H}^{\!-\!1} \mathbf{z}_2\!&\!\mathbf{z}_2^\top\mathbf{H}^{\!-\!\top}\!\mathbf{H}^{\!-\!1} \mathbf{z}_2\end{pmatrix}&=\!\frac{\sigma^2 \overline{\beta}^2}{\overline{s}^2\beta^2}\!\begin{pmatrix}
\mathbf{z}_1^\top \mathbf{z}_1  \!\!&  \!\!\mathbf{z}_1^\top \mathbf{z}_2 \\ \mathbf{z}_1^\top \mathbf{z}_2  \!\!& \!\! \mathbf{z}_2^\top \mathbf{z}_2 
\end{pmatrix}\!, \nonumber \\
\Rightarrow \mathbf{z}_i^\top \left(\overline{\mathbf{H}}^\top\overline{\mathbf{H}}-\frac{\sigma^2 \overline{\beta}^2}{\overline{s}^2\beta^2}\mathbf{I}_{3\times 3}\right)\mathbf{z}_j & = 0, \forall i,j \in [1,2],
\end{align}
\end{small}
%
where $\overline{\mathbf{H}}=\mathbf{H}^{-1}$. Assuming $\mathbf{H}$ to be normalized, that is, its second singular value to be 1, the relation between 3D points is given by $\phi(\mathbf{x}) = \mathbf{H} \phi(\overline{\mathbf{x}}) $. Using Eq.~\ref{eq:homography} yields $\overline{\beta} = \beta \overline{s}$. By writing $\mathbf{z}_i = [\mathbf{n}]_{\times}[\mathbf{h}_i]_\times \hat{\mathbf{x}}$, the above constraints further simplify to
\begin{equation}
\label{eq:recon_H}
[\mathbf{n}]_\times^\top (\overline{\mathbf{H}}^\top\overline{\mathbf{H}}-\sigma^2\mathbf{I}_{3\times 3})[\mathbf{n}]_\times = 0.
\end{equation}
%
Since $\alpha \mathbf{H}$ is equivalent to $\mathbf{H}$, we divide the above expression by $\sigma^2$ and write $\frac{1}{\sigma}\overline{\mathbf{H}}$ as $\overline{\mathbf{H}}$. This simplifies the above expressions to
%
\begin{equation}
\label{eq:final}
[\mathbf{n}]_\times^\top (\overline{\mathbf{H}}^\top\overline{\mathbf{H}}-\mathbf{I}_{3\times 3})[\mathbf{n}]_\times =[\mathbf{n}]_\times^\top \mathbf{S}[\mathbf{n}]_\times = 0.
\end{equation}

\parag{Degenerate cases.} The system of Eq.~\ref{eq:recon_H} holds as long as $\mathbf{S}$ is a non-null matrix, which means $\overline{\mathbf{H}}^\top \overline{\mathbf{H}} \neq \mathbf{I}_{3\times3}$.  Since $\overline{\mathbf{H}}$ is a planar homography, we write $\overline{\mathbf{H}}=\mathbf{R} 
+\frac{\mathbf{t}\mathbf{n}^\top}{d}$ where $\mathbf{R}$ rotation and $\mathbf{t}$ is translation. In case the relative motion between camera and object is purely rotational, $\overline{\mathbf{H}}^\top \overline{
\mathbf{H}} = \mathbf{I}_{3\times3}$ and the system~\eqref{eq:recon_H} does not hold. Another possibility is the mirror reflection about the plane, i.e. $\mathbf{t} = -2\mathbf{R}\mathbf{n}$ with $||\mathbf{t}||=2$ which is highly unlikely.

\parag{Affine stability.} Under affine imaging conditions, $h_{31}=h_{32}=0$ and $h_{33}=1$.
By making these changes, we see that $\mathbf{z}_i$ and $\mathbf{S}$ remain  non-null. Therefore, the system~\eqref{eq:recon_H} holds and we can obtain the solution to normals. 

\parag{Solution.} A solution to this system is obtained by homography decomposition~\cite{Malis07}. We give an overview of the solution here. We recommend reading~\cite{Malis07} for more details.

$\mathbf{S}={s_{ij}}$ is a symmetric matrix expressed in terms of $\mathbf{H}$ which can be numerically computed using $\eta$ and image observations $(\mathbf{x},\overline{\mathbf{x}})$. $\mathbf{T}$ in equation~\eqref{eq:CS_norm} shows a closed-form definition of $\mathbf{H}$. We write $\mathbf{n} = \begin{pmatrix}
n_1 & n_2 & n_3
\end{pmatrix}^\top$. Since $n_3 \neq 0$, we write $y_1 = \frac{n_1}{n_3}$ and $y_2 = \frac{n_2}{n_3}$ and expand the system~\eqref{eq:recon_H}. We obtain 6 constraints out of which, only 3 are unique. They are given by
\begin{align}
\label{eq:quad_recon}
\nonumber s_{33} y_2^2 - 2s_{23} y_2 + s_{22} &= 0 \\
\nonumber s_{33} y_1^2 - 2s_{13} y_1 + s_{11} &= 0 \\
s_{22} y_1^2 - 2s_{12} y_1 y_2 + s_{11} y_2^2 &= 0
\end{align}
By solving the first two quadratics, we obtain $y_1 = \dfrac{s_{13} \pm \sqrt{s_{13}^2-s_{33}s_{11}}}{s_{33}}$ and $y_2 =\dfrac{s_{23} \pm \sqrt{s_{23}^2-s_{33}s_{22}}}{s_{33}}$. We use the third expression to diambiguate the solutions. Thus, a closed form expression for the possible pair of normals is given by
\begin{align}
\label{eq:normal_sol}
\nonumber
&\mathbf{n}_a = \begin{pmatrix}
s_{13} + s\sqrt{s_{13}^2-s_{33}s_{11}}& s_{23} + \sqrt{s_{23}^2-s_{33}s_{22}}&s_{33}
\end{pmatrix}^\top\!, \\
\nonumber
&\mathbf{n}_b = \begin{pmatrix}
s_{13} - s\sqrt{s_{13}^2-s_{33}s_{11}}&s_{23} - \sqrt{s_{23}^2-s_{33}s_{22}}&s_{33}
\end{pmatrix}^\top\!, \\
&\text{where } s = sign(s_{23}s_{13}-s_{12}s_{33}).
\end{align}

\parag{Normal selection.} Using equation~\eqref{eq:k1k2}, the local depth derivatives $(k_1,k_2)$ at $\mathbf{X}$ are given by $\left(\frac{n_1}{n_3},\frac{n_2}{n_3}\right)$, $k_i=\frac{n_i}{u n_1 + vn_2 + n_3}$.
 From the solution~\eqref{eq:normal_sol}, we obtain two possible solutions to local depth derivatives
$(k_{1a},k_{2a})$ and $(k_{1b},k_{2b})$.
We pick the normal that minimizes the corresponding sum of squares of depth derivatives. Our chosen normal $\mathbf{n}_c$ is given by
\begin{equation}
\label{eq:nc}
\mathbf{n}_c = \begin{cases}
\mathbf{n}_a  & \text{ if } k_{1a}^2 + k_{2a}^2 \leq  k_{1b}^2 + k_{2b}^2 \\
\mathbf{n}_b  & \text{ otherwise } 
\end{cases}
\end{equation}
As shown in equation~\eqref{eq:homography},  $\overline{\mathbf{n}}$ is given by $\mathbf{H}^\top\mathbf{n}_c$.

\parag{Measure of degeneracy.} In case of degenerate conditions, the singular values $(\lambda
_1,\lambda_2,\lambda_3)$ of $\mathbf{H} $ are all unity. 
We use the ratio $\frac{\lambda_1}{\lambda_3}$ to quantify the degeneracy. Thus, we only reconstruct from $\mathbf{S}$, if $\frac{\lambda_1}{\lambda_3} > \tau$. We set $\tau = 1.2$. We put an upper limit $\tau = 10$ to ensure that the data is well-conditioned as we observed that a high value of $\tau$ leads to inaccuracies caused by measurement errors on $\eta$.

\section{Computing Normals from Multiple Images}
Let $\{\bx ^i_j\}, i\in [1,M], j\in[1,N]$, denote a set of $N$ point correspondences between $M$ images. Our goal is to find the 3D point $\bX^i_j$ and the normal $\mathbf{N}^i_j$ corresponding to each $\bx ^i_j$. 
Using equation~\eqref{eq:CS_norm}, we write the local homography for each point correspondence $\mathbf{H}^{ik}_j$ between image pairs $(i,k) \in [1,M], i \neq k$ using the warps $\eta$.Each local homography $\mathbf{H}^{ik}_j$ is normalized by dividing by their second singular value. We compute $\mathbf{Hc}^{ik}_j$ given by the ratio of first and third singular value. We compute normals for each local homography $\mathbf{Hc}^{ik}_j$ using equation~\eqref{eq:normal_sol} and pick a unique solution using equation~\eqref{eq:nc}. The solution on the reference and non-reference image is given by$\mathbf{N}_j^{kk}$ and $\mathbf{N}_j^{ki}$ respectively. For non-degenerate cases, where $\tau \in [1.2,10]$, we compute normals $N^i_j$ by taking the mean of $\mathbf{N}_j^{ik}$ computed over $k$ reference images. We obtain 3D point $\bX^i_j$ by integrating the normals on each surface using the method described in~\cite{Parashar19a}. We summarise Diff-NRSfM in algorithm~\ref{alg:diff}.

\begin{algorithm}
\SetAlgoLined
 \KwData{$\bx^i_j, \mathbf{H}^{ik}_j$ and $\mathbf{Hc}^{ik}_j$}
 \KwResult{ $\bX^i_j$ and $\mathbf{N}^i_j$}
 $\tau_{min} = 1.2$, $\tau_{max} = 10$ \;
 \For{ each reference image $k = [1,M]$}{
 \For{ each point $j= [1,N]$}{  
 \For{  images $i= [1,M], i \neq k$}{
 \eIf{$\mathbf{Hc}^{ik}_j > \tau_{min}$ and $\mathbf{Hc}^{ik}_j < \tau_{max}$}{
  Compute normals using~\eqref{eq:normal_sol}\;
  Pick a solution $\mathbf{N}_j^{kk}$ using~\eqref{eq:nc}\;
  Write $\mathbf{N}_j^{ik} = (\mathbf{Hc}^{ik}_j)^\top \mathbf{N}_j^{kk}$\;
 }
 { Set $\mathbf{N}_j^{ik}, \mathbf{N}_j^{kk}$ to zero\;
 }
 }
 }
 }
  \For{ each point $j= [1,N]$}{  
   \For{  images $i= [1,M]$}{
 Obtain $\mathbf{N}^i_j$ by averaging the non-zero normals in $\mathbf{N}^{ik}_j$\;
 }
 }
 \For{  images $i= [1,M]$}{
 Integrate $\mathbf{N}^i_j$ to obtain $\mathbf{X^i_j}$.
 }
 \caption{Diff-NRSfM}
 \label{alg:diff}
\end{algorithm}


